Clembench: Using Game Play to Evaluate Chat-Optimized Language Models as Conversational Agents

Recent work has proposed a methodology for the systematic evaluation of "Situated Language Understanding Agents"-agents that operate in rich linguistic and non-linguistic contexts-through testing them in carefully constructed interactive settings. Other recent work has argued that Large Language Models (LLMs), if suitably set up, can be understood as (simulators of) such agents. A connection suggests itself, which this paper explores: Can LLMs be evaluated meaningfully by exposing them to constrained game-like settings that are built to challenge specific capabilities? As a proof of concept, this paper investigates five interaction settings, showing that current chat-optimised LLMs are, to an extent, capable to follow game-play instructions. Both this capability and the quality of the game play, measured by how well the objectives of the different games are met, follows the development cycle, with newer models performing better. The metrics even for the comparatively simple example games are far from being saturated, suggesting that the proposed instrument will remain to have diagnostic value. Our general framework for implementing and evaluating games with LLMs is available at https://github.com/clembench .

==> per-game-results-discussion.tex <==
\subsection{Detailed Per-Game Results}

\das{
From mattermost: Could all game owners please do the following:
\begin{itemize}
    \item look at results broken down by dataset (e.g., simple / medium / hard instances), and extract high level descriptions? (E.g., "the results reflect our grouping of the datasets, in that for all experiments, the scores decrease with an increase in difficulty". Or something else, if that's not the case.)
    \item hunt for interesting, and ideally systematic, problems in episodes that were played with low success. And derive insights from that. E.g., "it appears that most player-pairs / models were not able to make use of the letter-based feedback"
    \item ideally, find some objective measure that backs this up. That is, make use of the other metrics besides the preferred one, to make points about the models. (Important to keep in mind: We're not evaluating the games so much (although indirectly we're also doing that, as instrument for evaluating the models), but rather we are interested in seeing differences between the models. Especially differences that we can see as differences in e.g. parameter count (3 to 3.5 to 4) or training regime.
\end{itemize}
}

\das{So, this ideally takes the form of additional tables, showing for each model the behaviour on the different subsets, and potentially using additional metrics specific to each game. (Or not; there are also metrics that drill into how well the game rules are followed, like the count of reprompting.) Basically, like the main table, except instead of different games, different subsets. This is the stuff you can then verbalise, possibly together with juicy examples.}

\das{Do the successful episodes look like human-played ones? Can you see what strategy lead to the results? Do the unsuccessful episodes look like what unlucky human players would also produce? Or do they show obvious shortcomings of the way the models play?}


Additional insight can be gained by looking at game-specific results.

\paragraph{Taboo}
\begin{itemize}
  \item For the claude and luminous models, all game plays are aborted, meaning they cannot follow the basic formatting rules or use a taboo word in their description.
  \item The GPT models have a varying number of aborts, davinci aborted roughly 3/4, 3.5 aborted almost half (43\%), 4 aborted roughly 1/4, meaning that we see improvement here with the more developed models.
  \item The same is true for wins: davinci can win very few games (3\%), 3.5 wins 17\%, 4 wins 2 thirds.
  \item Speed needs to be recomputed but there does not seem to be any effect of game mode (different word frequencies) for any of the model pairings 
  \item
\end{itemize}

\paragraph{Drawing}

\begin{itemize}
    \item \textit{3.5} has the highest played ratio but \textit{4} has the highest quality score. It means that \textit{4} struggles with following the rules but when it can do that it gets the best score. Also, the highest score across all games.

    \item The paired models 3.5/4 or 4/3.5 still can not combine the best of both worlds: higher played ratio with \textit{3.5} and quality score with \textit{4}.

    \item Similar observation as in other games: \textit{cl} and \textit{lm} are not able to follow the rules.
\end{itemize}

\paragraph{Reference}

\begin{itemize}
    \item five out of seven models get perfect played ratio where the lowest is \textit{3} and \textit{lm} has the same pattern, can not follow the rules.
    
    \item unlike in any other game, \textit{cl} gets the highest quality score.
\end{itemize}

\paragraph{Wordle}
The overall results indicate that except for GPT-4, other cLLM models tend to rely more on the clue (supplementary information provided to guess the word) rather than the guess feedback. However, giving higher priority to the guess feedback is essential as it helps eliminate words from consideration and adheres to a core strategy of the Wordle game. Here is a summary of the analysis conducted on the model's guessing strategies and response behavior.
\begin{itemize}
  \item Both Claudie and Luminous models provided guesses without offering any explanations for their guesses. Given the importance of guessing the word in gameplay, we included these games in the evaluation and scored them based on how closely the guessed word matched the target word.
  \item In the traditional Wordle variant, although all Luminous model plays consist of six guesses, the model consistently guessed the word "apple" (which was mentioned as an example in the prompt). This indicates its inability to accurately guess a word that adheres to the given rules. Similarly, majority games in the variant of Wordle with semantic clues and a critic were aborted due to the Luminous model's failure to respond with the guessed word in the correct format.
  \item In Claude's case, during traditional Wordle gameplay, all the plays exhausted their six attempts, and it appears that the guesses were made by not taking the guess feedback into consideration. This is evident from the use of incorrect letters in subsequent guesses, even after receiving the feedback. In the game variant with the clue, this behavior is enforced, allowing Claude to win 40\% of the games. In this variant, all the guesses are focused on the provided clue rather than on the feedback from previous guesses. However, the model stumbles when a critic is present, resulting in 50\% of games being aborted due to a failure to respond in the required format. Moreover, in the games it does manage to win, the focus remains on the clue rather than the critic's opinion.
  \item Among the GPT models, Davinci has the highest abort rate due to noncompliance with the guess response format, while GPT-4 successfully played all the games without aborting. GPT-3.5 comes in a close second.
  \begin{itemize}
    \item Davinci showcases a similar phenomenon to Claude in its focus on the clue rather than the feedback. This is evident through its explanations of why it is guessing a word and how it relates to the clue.
    \item While GPT-3.5 almost always responds in the expected format, its accuracy in guessing the correct word is often incorrect. The model explains its reasoning for selecting a word by considering past feedback, sometimes omitting certain letters due to their incorrectness. However, the guessed word still includes those incorrect letters. This highlights the model's inability to generate a word while adhering to omission rules, resulting in lower scores compared to the Davinci model.
    \item Among all the models, GPT-4 has the highest success rate in addition to the highest playing rate. It is the only model that shows positive (greater than 0) success rate for the traditional Wordle variant. Careful analysis of results indicate that while the model effectively handles feedback for the correct letters (right positions), it has difficulty in dealing with coorrect letters (wrong positions) and incorrect letters. Although the explanation states that a specific letter is correct but in the wrong position, the subsequent guesses continued to use those letters in the same positions instead of considering a change in position. This indicates model's shortcoming in adapting to the game strategy. In the Wordle variant with a critic, the model incorporates the critic's opinion to determine whether to retain or modify the guess. This approach leads to a higher success rate compared to other Wordle variants.   
  \end{itemize}
  
\end{itemize}

\paragraph{PrivateShared} \input{privateshared-game-resources/privateshared-eval}


==> taboo-game-resources/low_en_transcript.tex <==



{ \footnotesize  \setcounter{utterance}{1}
\setlength{\tabcolsep}{0pt}
\begin{supertabular}{c@{$\;$}|p{.15\linewidth}@{}p{.15\linewidth}p{.15\linewidth}p{.15\linewidth}p{.15\linewidth}p{.15\linewidth}}

    \# & $\;$A & \multicolumn{4}{c}{Game Master} & $\;\:$B\\
    \hline 

    \theutterance \stepcounter{utterance}  

    & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.9,0.9,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$\rangle$B]}  
	 You are playing a collaborative word guessing game in which you have to guess a target word that another player describes to you. [...]
	  } 
	   } 
	   } 
	 & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.9,0.9,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [A$\langle$GM]}  
	 [...] This is the target word that you need to describe and that the other player needs to guess:\\ \tt \\ \tt expedition\\ \tt \\ \tt Related words are:\\ \tt \\ \tt - journey\\ \tt - discovery\\ \tt - exploration\\ \tt \\
	  } 
	   } 
	   } 
	 & \\ 
 

    \theutterance \stepcounter{utterance}  

    & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.8,1,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [A$\rangle$GM]}  
	 CLUE: A trip taken for a specific purpose. 
	  } 
	   } 
	   } 
	 & & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & & \multicolumn{2}{p{0.3\linewidth}}{\cellcolor[rgb]{0.95,0.95,0.95}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$|$GM]}  
	 A trip taken for a specific purpose 
	  } 
	   } 
	   } 
	 & & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.9,0.9,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$\rangle$B]}  
	 CLUE: A trip taken for a specific purpose 
	  } 
	   } 
	   } 
	 & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{1,0.85,0.72}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$\langle$B]}  
	 GUESS: Journey 
	  } 
	   } 
	   } 
	  \\ 
 

    \theutterance \stepcounter{utterance}  

    & & & \multicolumn{2}{p{0.3\linewidth}}{\cellcolor[rgb]{0.95,0.95,0.95}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$|$GM]}  
	 journey 
	  } 
	   } 
	   } 
	 & & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.9,0.9,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [A$\langle$GM]}  
	 GUESS: journey 
	  } 
	   } 
	   } 
	 & \\ 
 

    \theutterance \stepcounter{utterance}  

    & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.8,1,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [A$\rangle$GM]}  
	 CLUE: A planned and organized trip with a specific goal in mind. 
	  } 
	   } 
	   } 
	 & & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & & \multicolumn{2}{p{0.3\linewidth}}{\cellcolor[rgb]{0.95,0.95,0.95}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$|$GM]}  
	 A planned and organized trip with a specific goal in mind 
	  } 
	   } 
	   } 
	 & & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{0.9,0.9,0.9}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$\rangle$B]}  
	 CLUE: A planned and organized trip with a specific goal in mind 
	  } 
	   } 
	   } 
	 & \\ 
 

    \theutterance \stepcounter{utterance}  

    & & & \multicolumn{4}{p{0.6\linewidth}}{\cellcolor[rgb]{1,0.85,0.72}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$\langle$B]}  
	 expedition 
	  } 
	   } 
	   } 
	  \\ 
 

    \theutterance \stepcounter{utterance}  

    & & & \multicolumn{2}{p{0.3\linewidth}}{\cellcolor[rgb]{0.95,0.95,0.95}{%
	\makecell[{{p{\linewidth}}}]{%
	  \tt {\tiny [GM$|$GM]}  
	 Game ends, because the response was invalid 
	  } 
	   } 
	   } 
	 & & \\ 
 

\end{supertabular}
}


==> taboo.tex <==
\paragraph{Game Description}

\das{As the first game, and one of the more straightforward ones (in terms of prompting), this could start with an almost complete transcript, showing the prompt (maybe with the one-shot example edited out (``[\dots]'') and picking an example where the second guesser turn is correct. This could be referenced in the text above describing the general schema; and it would also introduce notions that the later descriptions can refer to.}

In this game one player (the Describer) describes a target word for another player to guess (Guesser).
The Describer must explain the target word concept without using neither the word itself, nor a part of the word.
For example, when the target word is {\it flashlight}, the Describer cannot use the words {\it light or flash}.
After each incorrect guess by the Guesser, the Describer can add to his description.
The game ends when the Guesser guesses correctly or a maximum number of turns has been reached.

The game tests a cLLM's ability to describe concepts and give meaning definitions.
It also tests whether it can detect parts of words and its helpfulness in the game context.
For example, if a Describer does not alter or extend its initial description after an incorrect guess, we consider this unhelpful behavior.
On the opposite side, if a Guesser repeats an earlier guess, it has not understood the game goal well enough to make real progress at each turn.

\paragraph{Instantiation}

We instantiate this game by setting the maximum number of guesses to 3 and we use target words that vary according to their frequency.
We use an English word frequency list based on web data \cite{brants2006}\footnote{\url{https://www.kaggle.com/datasets/rtatman/english-word-frequency}} to derive a list of lemmatized content words from which we choose words from 3 levels of frequency:
We remove words with a frequency of less than 5 per 1 million tokens.
The remaining low-frequency words occur up $9.4$ times per 1 million tokens, the medium-frequency words occur up to $25.1$ times per 1 million tokens and the high-frequency tokens occur up to $12951.3$ times in 1 million tokens.
After a random selection from each frequency level, we manually ensure that the final word list does not contain inappropriate words such as vulgar language or proper names.
The final word lists contain 10 words each.
We use word frequency as a proxy for the difficulty of a game instance.

The players are each given their own prompts, as shown in Figure~\ref{fig:taboo_prompts}.
\input{taboo-game-resources/prompts.tex}

\paragraph{Evaluation}

We measure the following metrics at the episode-level (the example can be found in Figure~\ref{fig:taboo_example_1}):
\begin{enumerate}
  \item {\bf Success}: Whether or not the Guesser guessed the target word. In the example, success is $0$.
  \item {\bf Abort}: $1$ if any player did not follow the rules, and $0$ otherwise. In the example, abort is $1$.
  \item {\bf Speed}: How early the Guesser guessed the word as measured by the turn number in which the target was found. When the game was unsuccessful or aborted, as in the example, speed is the maximum number of turns+1 (4), so that smaller values signify better results.
\end{enumerate}


\begin{figure}
   \centering
   \input{taboo-game-resources/low_en_transcript}
   \caption{An example taboo episode that ends because the Guesser used an invalid response format.}
   \label{fig:taboo_example_1}
\end{figure}


==> wordle.tex <==
\paragraph{Game Description}
The popular word guessing game ``Wordle'' gained global attention, in which players are challenged to guess a five-letter word in six attempts.  After each guess, the player receives a feedback indicating which letters are in correct position, which letters are correct but in wrong position and which letters are incorrect to help them strategize their next guess. The objective of the game is to guess the target word using the fewest possible guesses, and the game ends when the player guesses correctly or exhausts all six attempts.

This game evaluates three key aspects of cLLM's capabilities. Firstly, it assesses how well the cLLM comprehends the game rules, which involves generating valid English words consisting of exactly five letters. Secondly, it measures how effectively cLLM uses guess feedback to generate its next guesses. Thirdly, it measures how quickly cLLM can guess the target word, if it succeeds.

In addition, we tested three different variations of the game to observe how the cLLM performs under different challenges. Below is a summary of these variations.

\subsubsection{Wordle (basic version)}
\paragraph{Game Description}
cLLM plays the roles of the ``player A'', %
and a deterministic wordle bot plays the role of ``player B''. Game begins by the game master prompting the player A to guess the target word~(as shown in Figure~\ref{fig:wordle_no_clue_no_critic_prompt_playerA}). The game master parses the player A's response and forwards it to the ``player B''~(as shown in Figure~\ref{fig:wordle_no_clue_no_critic_playerB}), which evaluates the closeness of guess word to the target word and returns the feedback. The game master sends the feedback to ``player A'' for the next guess and the cycle continues until the target word is guessed correctly or all the six attempts are exhausted. Please check appendix~\ref{sec:appendix_wordle_game_no_clue_no_critic_prompt}, for the complete flow of conversation between game master and the players.

\subsubsection{Wordle (+ Semantics-Based Clue)}
\paragraph{Game Description}

This is a Wordle variant, where the guesser (player A) gets a clue before starting guessing.

E.g., For the target word PRIDE, clue could be ``pack of lions''.

The primary aim of testing this variant is to evaluate the efficacy of Player A (role played by cLLM) in effectively utilizing the supplementary information provided by a clue to improve its guess of the target word. The clue serves as an aid to narrow down the possible word options. The success of the game depends on Player A's ability to integrate the clue with the guess\_feedback. Player A's explanation offers insights on how the cLLM links the clue phrase and the guess\_feedback. Please check appendix~\ref{sec:appendix_wordle_game_clue_no_critic_prompt}, for the complete flow of conversation between game master and the players.

\subsubsection{Wordle (+ Clue, + Critic)}
\paragraph{Game Description}

This game variant also begins with the guesser (Player A) who attempts to guess the target word based on a given clue. In contrast to other game variants, where the guessed word is immediately evaluated for its proximity to the target word, in this variant, the guess word and the clue are forwarded to another player known as the critic, for their opinion on the correctness of the guess. The critic responds with either agreement or disagreement, providing their rationale based on the information given. The critic's response is then relayed to the guesser, who can decide to stick with their initial guess or change it based on the feedback received. Please check appendix~\ref{sec:appendix_wordle_game_clue_critic_prompt}, for the complete flow of conversation between game master and the players.

This game variant helps to investigate the influence of the critic role in the guesser's performance and can lead to interesting possibilities in human-machine interaction, where the human can be aided by the cLLM as the critic. We tested the game using the same cLLM for both roles, as well as different cLLMs for each role, employing distinct prompts for each.


\paragraph{Instantiation}
In our experiments, we use a target list of 2,309 words\footnote{\label{wordle_target_words}\url{https://github.com/3b1b/videos/blob/master/_2022/wordle/data/possible_words.txt}} and a guess list of 12,953 words\footnote{\url{https://github.com/3b1b/videos/blob/master/_2022/wordle/data/allowed_words.txt}}. We also use New York Times crossword clues\footnote{\url{https://www.kaggle.com/datasets/darinhawley/new-york-times-crossword-clues-answers-19932021}} to retrieve clue phrases for our target words and word frequency information\footnote{\label{wordle_word_frequency}\url{https://www.kaggle.com/datasets/rtatman/english-word-frequency}} to categorize them. Out of the initial 2,309 target words, frequency details are not available for one word, and clues are not available for 39 words. These words are subsequently excluded from the experiments. The remaining 2,269 target words, are sorted based on their word frequency (descending frequency) and then divided them into three equal groups. The first group which contains high-frequency words, has a total of 756 words. The second group, consisting of words with medium frequency, also contains 756 words. Finally, the third group, which contains low-frequency words, has a total of 757 words. To evaluate our methodology, we chose (random seed: 42) 10 words from each frequency group, resulting in a total of 30 target words for evaluation purposes.

\paragraph{Evaluation}
For each episode, we record the number of guesses made by the guesser. If the guesser correctly guessed the word in six or fewer attempts, the game is counted as a success. If the guesser exhausted all the six attempts, the game is counted as a fail. Of the successful games, the average number of guesses took to guess the word is computed. For all the games, we also measured how close the guess gets to target word with each turn and how many times the guesser repeats the same guess. For the episodes, where critic is available we count how many times the guesser changed the guess based on critic's opinion.  The following are the metrics measured for each episode.
\begin{enumerate}
  \item {\bf Success Rate}: Measures whether the guesser guessed the target word or not
  \item {\bf Rank}: Computes how quickly the guesser guessed the word.
  \item {\bf Closeness}: Determines how effectively the guesser utilizes the guess feedback.
  \item {\bf Repetition-Guesser}: Assess how often the guesser repeated a guess.
  \item {\bf Change-Of-Opinion-Guesser}: Calculates the number of times guesser changing/retaining the guess
\end{enumerate}

\input{wordle-game-resources/high_freq_clue_critic_short_transcript}



